Improving Multi-Task Deep Neural Networks via Knowledge Distillation for Natural Language Understanding

This paper explores the use of knowledge distillation to improve a Multi-Task Deep Neural Network (MT-DNN) (Liu et al., 2019) for learning text representations across multiple natural language understanding tasks. Although ensemble learning can improve model performance, serving an ensemble of large DNNs such as MT-DNN can be prohibitively expensive. Here we apply the knowledge distillation method (Hinton et al., 2015) in the multi-task learning setting. For each task, we train an ensemble of different MT-DNNs (teacher) that outperforms any single model, and then train a single MT-DNN (student) via multi-task learning to \emph{distill} knowledge from these ensemble teachers. We show that the distilled MT-DNN significantly outperforms the original MT-DNN on 7 out of 9 GLUE tasks, pushing the GLUE benchmark (single model) to 83.7\% (1.5\% absolute improvement\footnote{ Based on the GLUE leaderboard at https://gluebenchmark.com/leaderboard as of April 1, 2019.}). The code and pre-trained models will be made publicly available at https://github.com/namisan/mt-dnn.

==> model.tex <==
\section{MT-DNN-1}
\label{sec:mt-dnn-1}

\subsection{Preliminaries}
\label{subsec:prelim}
In this work, our multi-task model combines classification, regression and pair-wise ranking tasks, which are summerised in Table~\ref{tab:task}. We briefly introduce the definition of each task as follows: 
\begin{table}[htb!]
	\begin{center}
		\begin{tabular}{@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}c@{\hskip1pt}|@{\hskip1pt}c@{\hskip1pt}|@{\hskip1pt}c}
			\hline \bf Input &Classification&Regression &Ranking\\ \hline \hline
			single sentence &$\checkmark$&& \\
			pairwise text &$\checkmark$&$\checkmark$&$\checkmark$ \\ \hline
		\end{tabular}
	\end{center}
	\lgspace
	\caption{Summary of tasks in our multi-task framework.
	}
	\label{tab:task}
\lgspace
\end{table}
\begin{figure}[!t]
\centering
\adjustbox{trim={.065\width} {.01\height} {.05\width} {.01\height},clip}
{\includegraphics[scale=0.7]{mtl_model}}
\caption{Model architecture.}
\label{fig:mtl_model} 
\end{figure}

\begin{figure}[!t]
\centering
\adjustbox{trim={.05\width} {.01\height} {.05\width} {.01\height},clip}
{\includegraphics[scale=0.7]{mtl_model_v2}}
\caption{Model architecture version 2.}
\label{fig:mtl_model_v2} 
\end{figure}

\textbf{Task definition}

\textbf{Objective}

\textbf{Single classification}
\xiaodl{Need to cluster different tasks..}

\textbf{Sentence-pair classification}: given a pair of sentence, $(S_1, S_2)$, the model predicts a label indicating the relation of this pair of sentences: $P(C|S_1, S_2)$. For example, natural language inference is a typical instance of the sentence-pair classification task: a premise and a hypothesis are denoted by $S_1$ and $S_2$, respectively; the label, $C$, belongs one of three relations (\textit{contradiction}, \textit{neutral} and \textit{entailment}). 

\textbf{Regression}


\textbf{Pair-wise Ranking}
\begin{algorithm}[ht!]
 \SetAlgoLined
Initialize model parameters $\Theta$ randomly  \\
Set M \quad\textit{//the number of updates for the shared layer} \\
%\textit{Counter} = 0\\
 \For{$iteration$ in $0 ... \infty$}{
 	 %1. \textit{Counter} += 1\\
     1. Pick a task $t$ randomly \\
     2. Pick sample(s) from task $t$, i.e., \\
     \hspace{0.4cm}$(Q,C=\{0,1\})$ for classification \\
     \hspace{0.4cm}$(Q, D)$ for ranking\\
     3. Compute loss: $L(\Theta)$, i.e.,\\
     \hspace{0.4cm} the \textit{cross-entropy} for classification \\
     \hspace{0.4cm} the ranking loss for ranking\cite{learning-to-rank2005burges}\\

     4. Compute gradient: $\nabla(\Theta)$ \\
     5. Update model: $\Theta = \Theta - \epsilon \nabla(\Theta)$ \quad\textit{}
     % \eIf{Counter $<$ M}{
  	 %5. Update model: $\Theta = \Theta - \epsilon \nabla(\Theta)$ \quad\textit{//update both $\Theta^s$ and $\Theta^t$} \\
   %}{
   	% 6. Update model: $\Theta^t = \Theta^t - \epsilon \nabla(\Theta^t)$ 
  %}
 }
 \caption{\label{algo:mtdnn} Training a Multi-task model.}
 \algorithmfootnote{Note that $\Theta$ denotes the model parameters. \textcolor{red}{TODO: update alg based on task defination.}}
\end{algorithm}

==> related.tex <==
\section{Acknowledgements}
\label{sec:akn}

We would like to thanks Jade Huang from Microsoft for her generous help on this work.

==> tasks.tex <==
\section{Tasks}
\label{sec:tasks}

The MT-DNN model combines four types of NLU tasks: single-sentence classification, pairwise text classification, text similarity scoring, and relevance ranking. For concreteness, we describe them using the NLU tasks defined in the GLUE benchmark as examples. 
%The GLUE tasks are summarized in Table 1.

\paragraph{Single-Sentence Classification:} 
Given a sentence\footnote{In this study, a sentence can be an arbitrary span of contiguous text or word sequence, rather than a linguistically plausible sentence.}, the model labels it using one of the pre-defined class labels. For example, the \textbf{CoLA} task  is to predict whether an English sentence is grammatically plausible. The \textbf{SST-2} task is to determine whether the sentiment of a sentence extracted from movie reviews is positive or negative.

\paragraph{Text Similarity:}
This is a regression task. Given a pair of sentences, the model predicts a real-value score indicating the semantic similarity of the two sentences. \textbf{STS-B} is the only example of the task in GLUE. 

\paragraph{Pairwise Text Classification:} 
Given a pair of sentences, the model determines the relationship of the two sentences based on a set of pre-defined labels. 
For example, both \textbf{RTE} and \textbf{MNLI} are language inference tasks, where the goal is to predict whether a sentence is an \emph{entailment}, \emph{contradiction}, or \emph{neutral} with respect to the other. 
% \textbf{WNLI} is a natural language inference task that requires commonsense reasoning. But as noted in the GLUE webpage \footnote{https://gluebenchmark.com/faq}, there are issues in the dataset, and every submitted system has performed same or worse than the majority voting baseline whose accuracy is 65.1. MT-DNN also achieves the accuracy of 65.1, making WNLI the only GLUE task where MT-DNN does not create a new state of the art result.
\textbf{QQP} and \textbf{MRPC} are paraphrase datasets that consist of sentence pairs. The task is to predict whether the sentences in the pair are semantically equivalent.

\paragraph{Relevance Ranking:}
Given a query and a list of candidate answers, the model ranks all the candidates in the order of relevance to the query. 
\textbf{QNLI} is a version of Stanford Question Answering Dataset \citep{rajpurkar2016squad}. 
The task involves assessing whether a sentence contains the correct answer to a given query. 
Although QNLI is defined as a binary classification task in GLUE, in this study we formulate it as a pairwise ranking task, where the model is expected to rank the candidate that contains the correct answer higher than the candidate that does not. 
We will show that this formulation leads to a significant improvement in accuracy over binary classification.

%is derive from the Stanford Question Answering Dataset \citep{rajpurkar2016squad}, and consists  which has been converted to a binary classification task in GLUE. A query-candidate-answer pair is labeled as positive if the candidate contains the correct answer to the query, and negative otherwise. In this study, however, we formulate QNLI as a pairwise ranking task, where the model is expected to rank the candidate that contains the correct answer higher than the candidate that does not. We will show that our formulation leads to a significant improvement in accuracy over binary classification. 


\begin{algorithm}[ht!]
 \SetAlgoLined
\textbf{P}re-train teacher models for all tasks \\  
\textbf{I}nitialize model parameters $\Theta$ randomly.  \\
\textbf{P}re-train the shared layers (i.e., the lexicon encoder and the transformer encoder). \\
\textbf{S}et the max number of epoch: $epoch_{max}$.
\textit{//Prepare the data for $T$ tasks.}\\
\For{$t$ in $1,2,...,T$ }
{
    Pack the dataset $t$ into mini-batch: $D_t$.
}

 \For{$epoch$ in $1,2,...,epoch_{max}$}{
     1. Merge all the datasets: $D =D_1 \cup D_2 ... \cup D_T$ \\
     2. Shuffle $D$ \\
     \For{$b_t$ in D}{
        \textit{//$b_t$ is a mini-batch of task $t$.} \\
         $\hat{y_t}$ = $Teacher_t(b_t)$ \\
     3. Compute loss : $L(\Theta)$ \\
        \hspace{0.3cm} $L(\Theta)=$ Eq.~\ref{eqn:cross-entropy-loss} + Eq.~\ref{eqn:kl} for classification \\
        \hspace{0.3cm} $L(\Theta)=$ Eq.~\ref{eqn:msq-loss} for regression \\
        \hspace{0.3cm} $L(\Theta)=$ Eq.~\ref{eqn:ranking-loss} + Eq.~\ref{eqn:kl} for ranking \\
     4. Compute gradient: $\nabla(\Theta)$ \\
     5. Update model: $\Theta = \Theta - \epsilon \nabla(\Theta)$ \\
     }
 }
 \caption{\label{algo:kdmtdnn} Training a {\NMNAME} model.}
\end{algorithm} 

